Unveiling frequency-dependent eclipsing in spider millisecond pulsars using broadband polarization observations with the Parkes

This study presents an orbital phase-dependent analysis of three black widow spider millisecond pulsars (BW MSPs), aiming to investigate the magnetic field within the eclipse environment. The ultra-wide-bandwidth low-frequency receiver (UWL) of the Parkes 'Murriyang' radio telescope is utilised for full polarisation observations covering frequencies from 704-4032 MHz. Depolarisation of pulsed emission is observed during the eclipse phase of three BW MSPs namely, J0024-7204J, J1431-4715 and PSR J1959+2048, consistent with previous studies of other BW MSPs. We estimated orbital phase dependent RM values for these MSPs. The wide bandwidth observations also provided the constraints on eclipse cutoff frequency for these BW MSPs. For PSR J0024-7204J, we report temporal variation of the eclipse cutoff frequency coupled with changes in the electron column density within the eclipse medium across six observed eclipses. Moreover, the eclipse cutoff frequency for PSR J1431-4715 is determined to be 1251 $\pm$ 80 MHz, leading to the conclusion that synchrotron absorption is the primary mechanism responsible for the eclipsing. Additionally, for PSR J1959+2048, the estimated cutoff frequency exceeded 1400 MHz, consistent with previous studies. With this investigation, we have doubled the sample size of BW MSPs with orbital phase-resolved studies allowing a better probe to the eclipse environment.

==> table1.tex <==
\begin{table*}[!htb]
\begin{center}
\caption{Summary of the observations$^{\dagger}$}
\label{tab:Table1}
\vspace{0.3cm}
\label{discovery}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l}
\hline
Pulsar name     & P$^{a}$ & DM$^{b}$ & $P_{b}^{c}$& Proposal code & Date & $T_{int}^{d}$ & OP$^{e}$ & $T_{sub}^{f}$\\
     & (ms)& ($pc~cm^{-3}$)& \textbf{(hrs)}& & & (hrs) &  & (s)\\
 
\hline
J0024$-$7204J   &2.101 &24.59& 2.8 &P1078$^{g}$ &16$-$08$-$2020 & 5.0 &  0.22$-$1.98$^{*}$ & 30\\
&&& & &27$-$01$-$2021 & 3.3 &    0.49$-$1.62$^{*}$  & 30  \\
 
&&&  & P1006 & 29$-$05$-$2019  & 3.6 &     0.39$-$1.68$^{*}$  & 20 \\
  
&&&   & & 08$-$07$-$2019 &  3.1 &    0.20$-$1.27$^{*}$  & 20 \\
&&&    & & 14$-$07$-$2019 & 2.8 &   0.97$-$1.94$^{*}$  & 20   \\
\hline
J1431$-$4715  &2.012&59.35&10.7&P789& 23$-$11$-$2018  & 3.6 &  0.62$-$0.94  & 20   \\
 &&& && 30$-$11$-$2018 &  0.4 &  0.40$-$0.45   &   20  \\
  &&&  && 08$-$12$-$2018 & 0.7 &   0.96$-$0.00      & 30  \\
   &&&   && 13$-$02$-$2019 & 0.4 &  0.07$-$0.26  & 30         \\
   &&&     && 27$-$04$-$2019 & 1.2 &   0.81$-$0.93   & 10      \\
   &&&       && 07$-$06$-$2019 & 1.6 & 0.28$-$0.42    &  10     \\
\hline


J1959$+$2048 &1.607&29.11& 9.1& P1078$^{g}$ & 06$-$10$-$2020  &2.4 &0.07$-$0.32 & 30  \\
&&&  & & 16$-$10$-$2020    & 2.8 & 0.12$-$0.43  & 30 \\
&&&  && 10$-$02$-$2021  & 3.1  & 0.17$-$0.51 & 30 \\
   
&&&     & & 27$-$01$-$2021  & 2.8   & 0.03$-$0.35 & 30 \\
\hline


\end{tabular}
\end{center}
$^{a}$: Spin period of the pulsar; $^{b}$: Dispersion measure; $^{c}$: Orbital period of the pulsar; $^{d}$: Total integration time; $^{e}$: Orbital phase covered; $^{f}$: Subintegration length; $^{g}$: Data for P1078 is acquired by some of the authors of this paper; $^{*}$: 1 in front of the orbital phase represents the orbital phase of next consecutive orbit; $^{\dagger}$: Publicly available Parkes UWL data, at CSIRO data archive

\vspace{1cm}
\end{table*}

==> table3.tex <==
\begin{table*}[hbt!]
\begin{center}
\caption{Table listing the cutoff frequency values for multiple observing epochs along with the corresponding electron column density in the eclipse medium.}
\label{tab:Table3}
\vspace{0.3cm}
\label{table2}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Pulsar name   & Date & Cutoff frequency($\nu_{c}$)& Eclipse orbital phase$^{a}$ & $N_{e}^{b}$ & Frequency$^{c}$\\
   &  & (MHz)&  & $(cm^{-2})$ & (MHz)\\
\hline
J0024$-$7204J   & 16$-$08$-$2020 & $<$ 734 & 0.22$-$0.26& $3\times 10^{16}$ & 734$-$1107 \\
 & 27$-$01$-$2021 & $<$ 1911 & 0.22$-$0.26& $4\times 10^{16}$& 1911$-$2221\\
  & 29$-$05$-$2019 & $<$ 1232 & 0.22$-$0.26&$5\times 10^{16}$& 1232$-$1655\\
   & 08$-$07$-$2019$^{1}$ & $<$ 734 & 0.18$-$0.21& $1\times 10^{16}$ & 734$-$1107\\
   & 08$-$07$-$2019$^{2}$ & $<$ 734 & 0.18$-$0.21 &$2\times 10^{16}$& 734$-$1107\\
    & 14$-$07$-$2019 & $>$ 1581 &0.22$-$0.26 &$4\times 10^{16*}$& 1251$-$1581\\
\hline
J1431$-$4715 &13$-$02$-$2019 & 1251 $\pm$ 80& 0.22$-$0.25&$9\times 10^{17*}$&1251$-$1600\\
     &07$-$06$-$2019 & 1251$\pm$ 80 & 0.28$-$0.30 &$9\times 10^{17*}$&1251$-$1600\\
\hline
J1959$+$2048 & 06$-$10$-$2020 & $>$ 1424 &0.23$-$0.26 &$4 \times 10^{16*}$&734$-$1107\\
 & 10$-$02$-$2021 & $>$ 1581  & 0.23$-$0.26&$3 \times 10^{17*}$&734$-$1107\\
  & 16$-$11$-$2020 & $>$ 1424 & 0.23$-$0.26&$5 \times 10^{16*}$&734$-$1107\\
   & 27$-$01$-$2021 & $>$ 1424 & 0.23$-$0.26&$1 \times 10^{17*}$&734$-$1107\\

\hline



\end{tabular}
\end{center}
$^{a}$: The orbital phase range averaged to determine the eclipse cutoff frequency.\\
$^{b}$: The maximum \textbf{electron column density} in the eclipse medium.\\
$^{c}$: Frequency chunk that has been considered to find the maximum value of $N_{e}$ in the eclipse medium.\\
$^{*}$: The epochs where only the limit on the $N_{e}$ is known.\\
$^{1}$: 1st orbit \\
$^{2}$: 2nd orbit \\


 

\vspace{1cm}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
